ICF-SRSR: Invertible scale-Conditional Function for Self-Supervised Real-world Single Image Super-Resolution

Single image super-resolution (SISR) is a challenging ill-posed problem that aims to up-sample a given low-resolution (LR) image to a high-resolution (HR) counterpart. Due to the difficulty in obtaining real LR-HR training pairs, recent approaches are trained on simulated LR images degraded by simplified down-sampling operators, e.g., bicubic. Such an approach can be problematic in practice because of the large gap between the synthesized and real-world LR images. To alleviate the issue, we propose a novel Invertible scale-Conditional Function (ICF), which can scale an input image and then restore the original input with different scale conditions. By leveraging the proposed ICF, we construct a novel self-supervised SISR framework (ICF-SRSR) to handle the real-world SR task without using any paired/unpaired training data. Furthermore, our ICF-SRSR can generate realistic and feasible LR-HR pairs, which can make existing supervised SISR networks more robust. Extensive experiments demonstrate the effectiveness of the proposed method in handling SISR in a fully self-supervised manner. Our ICF-SRSR demonstrates superior performance compared to the existing methods trained on synthetic paired images in real-world scenarios and exhibits comparable performance compared to state-of-the-art supervised/unsupervised methods on public benchmark datasets.

==> macro.tex <==
\newcommand{\sanghyun}[1]{\textcolor{blue}{\textbf{Sanghyun}: #1}}

\renewcommand{\eg}{\emph{e.g.}}
\renewcommand{\ie}{\emph{i.e.}}
\renewcommand{\etal}{\emph{et al.}}

==> sections/figures/realsr.tex <==
\begin{figure*}
     \captionsetup[subfigure]{aboveskip=1pt}
     \centering
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/5/LR_027.png.jpg}
         \label{fig:loss_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/5/realsr_027.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/5/ikc_027.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/5/zssr_027.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/5/Ours_027_4.png.jpg}
         \label{fig:loss_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/5/HR_027.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \\
     \vspace{-4mm}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/6/LR_003.png.jpg}
         \label{fig:loss_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/6/realsr_003.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/6/IKC_003.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/6/zssr_003.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/6/Ours_003.png.jpg}
         \label{fig:loss_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/nikon/6/HR_003.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \\
     \vspace{-4mm}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/8/LR_04.png.jpg}
         \label{fig:loss_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/8/realsr_04.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/8/ikc_04.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/8/zssr_04.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/8/IMF_04_4.png.jpg}
         \label{fig:loss_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/8/HR_04.png.jpg}
         \label{fig:loss_b}
     \end{subfigure}
    \\
     \vspace{-4mm}
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/5/LR_46.png}
         \caption*{Input}
         \label{fig:loss_a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/5/realsr_46.png}
         \caption*{LP-KPN~\cite{cai2019toward}}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/5/ikc_46.png}
         \caption*{IKC~\cite{gu2019blind}}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/5/ZSSR_046.jpg}
         \caption*{ZSSR~\cite{shocher2018zero}+~\cite{bell2019blind}}
         \label{fig:loss_b}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/5/Ours_3.png.jpg}
         \caption*{\textbf{ICF-SRSR}~(Ours)}
         \label{fig:loss_b}
     \end{subfigure}   
     \hfill
     \begin{subfigure}[b]{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/realsr/canon/5/HR_46.png}
         \caption*{GT}
         \label{fig:loss_b}
     \end{subfigure}
     %\vspace{-2mm}
        \caption{\textbf{Qualitative comparisons on a real-world dataset.} 
        %
        We visualize the super-resolution results for the images captured by each Nikon~(first and second rows) and Canon~(third and fourth rows) camera. 
        %
        We compare our self-supervised method ICF-SRSR with the supervised method LP-KPN~\cite{cai2019toward} and the unsupervised method ZSSR~\cite{shocher2018zero}+~\cite{bell2019blind} trained on the RealSR-V3~\cite{cai2019toward} dataset and the supervised method IKC~\cite{gu2019blind} trained on synthetic dataset DIV2K~\cite{agustsson2017ntire} for scale $\times4$.}
        \label{fig:realsr}
        \vspace{-4mm}
\end{figure*}     




